Flat'n'Fold: A Diverse Multi-Modal Dataset for Garment Perception and Manipulation

We present Flat'n'Fold, a novel large-scale dataset for garment manipulation that addresses critical gaps in existing datasets. Comprising 1,212 human and 887 robot demonstrations of flattening and folding 44 unique garments across 8 categories, Flat'n'Fold surpasses prior datasets in size, scope, and diversity. Our dataset uniquely captures the entire manipulation process from crumpled to folded states, providing synchronized multi-view RGB-D images, point clouds, and action data, including hand or gripper positions and rotations. We quantify the dataset's diversity and complexity compared to existing benchmarks and show that our dataset features natural and diverse manipulations of real-world demonstrations of human and robot demonstrations in terms of visual and action information. To showcase Flat'n'Fold's utility, we establish new benchmarks for grasping point prediction and subtask decomposition. Our evaluation of state-of-the-art models on these tasks reveals significant room for improvement. This underscores Flat'n'Fold's potential to drive advances in robotic perception and manipulation of deformable objects. Our dataset can be downloaded at https://cvas-ug.github.io/flat-n-fold

==> table_comparison_bkp.tex <==
\begin{table*}
\centering
\caption{Comparative Analysis with Other Datasets, * denotes that only the segment of the dataset related to deformable objects is selected.\lp{need to fill the numbers}\lp{double-check semantic state est. maybe both human and robot} \pmh{2212 for ours?} \pmh{`Agent' instead of `Cat'?} \pmh{narrow the columns (e.g. abbreviate things further), there's lots of wasted space}}
\resizebox{1\textwidth}{!}{\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
Dataset &  Agent  & Exp. Setting      & Garment Cat.        & \#Garments    &\#Seq. &Seq. Length  & \#Frame       & Deform. & Task     & Vis. Info & Hum. Action  & Ann. & Total Hrs.           \\  \midrule

VideoFolding~\cite{DBLP:journals/ijrr/VerleysenBw20} & Human      & Real        & 2          & (need fill)        & 1000        & Long & 304k & Large & Flatten\&Folding  & Multi-view RGBD & x   & Arm keypoint   &  8.5h \\

DeepDeform~\cite{DBLP:conf/cvpr/BozicZTN20} & Human  & Real        & 1         & (need fill) & 400        & Short & 39k & Mild & move  & Single-view RGBD & x  & Sparse keypoint   & (need fill) \\

Semantic State Est.~\cite{DBLP:journals/corr/abs-2203-11647}& Human     & Real         & 1          & 18        & (need fill)         & Short & 33.6K & Mild & Pick-up\&Folding  & RGB & x   & Cloth semantic state  & (need fill)\\

Garment Tracking~\cite{DBLP:conf/cvpr/XueXZTLDYL23} & Human    & Virtual        & 4          & (need check)    &(need fill)     & Long         & 790k & Large & Flatten\&Folding & Rendered Multi-view RGBD  & (need fill) & Garment\&Hand pose & (need fill)    \\

VR~\cite{DBLP:conf/ccia/Boix-GranellFT22} & Human     & Virtual        & 3     & 3         & 60         & Short & (need fill)- & Mild & Folding  & (need fill) & (need fill)   & (need fill)   & (need fill) \\ \midrule

Roboturk*~\cite{DBLP:conf/iros/MandlekarBSTGZG19} & Robot     & Real        & 3         & 3        & 920        & Medium & (need fill) & Mild & Flatten  & Multi-view RGBD & (need fill)   & (need fill) & $\sim$33h \\ \midrule

MIME*~\cite{DBLP:conf/corl/SharmaMPG18} & Human\&Robot     & Real         & 1          & 3(need check)         & (need fill)         & Short & (need fill) &Tiny & Wipe(no manipulation)  & Single-view RGBD & x   & (need fill)   &  (need fill)\\ \midrule

\textbf{Flat'n'Fold (ours)} & \textbf{Human\&Robot}    & \textbf{Real}        & \textbf{9}         & \textbf{46}         & \textbf{2212}         & \textbf{Long} & \textbf{$\sim$1600k} & \textbf{Large} & \textbf{Lifting, Flatten\&Folding}  & \textbf{Multi-view RGBD\&Pointcloud} & \checkmark  & \textbf{Grasping point\&time}  & \textbf{$>$100h}\\ 
\bottomrule
\end{tabular}}
\label{tab:Compare}
\end{table*}
